What is Missing? Explaining Neurons Activated by Absent Concepts

Explainable artificial intelligence (XAI) aims to provide human-interpretable insights into the behavior of deep neural networks (DNNs), typically by estimating a simplified causal structure of the model. In existing work, this causal structure often includes relationships where the presence of a concept is associated with a strong activation of a neuron. For example, attribution methods primarily identify input pixels that contribute most to a prediction, and feature visualization methods reveal inputs that cause high activation of a target neuron - the former implicitly assuming that the relevant information resides in the input, and the latter that neurons encode the presence of concepts. However, a largely overlooked type of causal relationship is that of encoded absences, where the absence of a concept increases neural activation. In this work, we show that such missing but relevant concepts are common and that mainstream XAI methods struggle to reveal them when applied in their standard form. To address this, we propose two simple extensions to attribution and feature visualization techniques that uncover encoded absences. Across experiments, we show how mainstream XAI methods can be used to reveal and explain encoded absences, how ImageNet models exploit them, and that debiasing can be improved when considering them.

==> figures/reichardt_experiment/reichardt_barplot.tex <==
    \begin{tikzpicture}[every node/.style={font=\sffamily}]
    \sffamily
    \scriptsize
\def\yscale{0.0001}
\def\ticklabely{0.00cm};
\def\setuponey{0.4};
\def\setuptwoy{0.0};

\def\myxmin{0};
\def\myxmax{2};
\def\myymin{-0.05};
\def\myymax{+0.2};

\def\centergroupone{0.5};
\def\centergrouptwo{1.5};
\def\centergroupthree{2.5};
\def\centergroupfour{3.5};
\def\centergroupfive{4.5};
\def\centergroupsix{5.5};
\def\centergroupseven{6.5};

\def\bardistance{0.3};
\def\barwidth{0.225};
\def\mymarkeroffsety{0.05}
    
\begin{axis}[
    axis lines=middle,
    xmin=\myxmin-0.55, xmax=\myxmax,
    ymin=\myymin-0.07, ymax=\myymax+0.07, %
    xtick=\empty, ytick=\empty,
    axis line style={draw=none},
    tick style={draw=none},
    height=3.3cm, 
    width=3.5cm,
]

\draw[-] (\myxmin,\myymin-0.0015) -- (\myxmin,0.2+0.001);
\draw[-] (\myxmin,1.45) -- (\myxmin,1.45) node[xshift=-0.7cm, anchor=center, rotate=90] {\scriptsize QUBA Score};
\draw[-] (\myxmin,\myymin) -- (\myxmax,\myymin);


\draw[-] (\myxmin,0.0) -- (\myxmin-0,0.00) node[left=\ticklabely,xshift=-0.2em] {\tiny 0};
\draw[-] (\myxmin,0.2) -- (\myxmin-0,0.2) node[left=\ticklabely,xshift=-0.2em] {\tiny 0.2};

\draw[-] ([yshift=-0.25cm]+1.0,\myymin) -- ([yshift=0.cm]+1.0,\myymin);


\draw[-] (\centergroupone,\myymin) -- (\centergroupone,\myymin) node[below=\ticklabely,yshift=-0.2em] {\tiny {class 1}};
\draw[-] (\centergrouptwo,\myymin) -- (\centergrouptwo,\myymin) node[below=\ticklabely,yshift=-0.2em] {\tiny {class 2}};




\draw[fill=colorSchemeOne, draw=colorSchemeOne!100] (\centergroupone-0.5*\bardistance-\barwidth/2,0+0.001) rectangle (\centergroupone-0.5*\bardistance+\barwidth/2,0.0769);

\draw[-, opacity=0] (\centergroupone-0.5*\bardistance,0.12-0.046) -- (\centergroupone-0.5*\bardistance,0.12+0.026) node[xshift=+0.8em, yshift=+0.0em, color=colorSchemeOne, opacity=1.0] {\tiny {output 1}};


\draw[fill=colorSchemeTwo, draw=colorSchemeTwo!100] (\centergroupone+0.5*\bardistance-\barwidth/2,0+0.001) rectangle (\centergroupone+0.5*\bardistance+\barwidth/2,0.0385);

\draw[-, opacity=0] (\centergroupone+0.5*\bardistance,0.12+0.046) -- (\centergroupone+1.9*\bardistance,0.12-0.042) node[xshift=-0.0em, yshift=0.3em, color=colorSchemeTwo, opacity=1.0] {\tiny {output 2}};



\draw[fill=colorSchemeOne, draw=colorSchemeOne!100] (\centergrouptwo-0.5*\bardistance-\barwidth/2,0+0.001) rectangle (\centergrouptwo-0.5*\bardistance+\barwidth/2,0.0+0.0011);

\draw[fill=colorSchemeTwo, draw=colorSchemeTwo!100] (\centergrouptwo+0.5*\bardistance-\barwidth/2,0+0.001) rectangle (\centergrouptwo+0.5*\bardistance+\barwidth/2,0.0769);











\draw[-] (\myxmin,\myymin) -- (\myxmax,\myymin);

\draw[very thin, -, draw opacity=0.5] (\myxmin,0.2) -- (\myxmax,0.2);
\draw[very thin, -, draw opacity=0.5] (\myxmin,0.0) -- (\myxmax,0.0);
\draw[very thin, -, draw opacity=0.5] (\myxmax,-0.05) -- (\myxmax,0.2);

\end{axis}





    \end{tikzpicture}


==> figures/reichardt_experiment/reichardt_lenet.tex <==
\begin{tikzpicture}[scale = 0.75]%
    \sffamily
    \scriptsize

    \colorlet{layergray2}{gray!60!black}{0.5}
    \colorlet{layergray1}{black!15}{0.5}
    \def\layersep{2.85}  %
    \def\layerwidth{1.25} %
    \def\layerheight{1.25}  %
    \def\depth{-1.1}      %
    \def\shift{-0.6}      %
    \def\filtersize{0.25};
    \def\xConvOneOne{0.0};
    \def\yConvOneOne{0.0};
    \def\xConvOneTwo{0};
    \def\yConvOneTwo{\layerwidth-\filtersize-\filtersize-0.02};
    \def\xConvTwoOne{0.0};
    \def\yConvTwoOne{0.0};
    \def\xConvTwoTwo{0.0};
    \def\yConvTwoTwo{\layerwidth-\filtersize-\filtersize-0.02};

    \def\ConvOneOneTarget{(\layersep-1 * \shift, 0+0.125, -1 * \depth)};
    \def\ConvOneTwoTarget{(\layersep-0 * \shift, 0+1.225, -0 * \depth)};
    \def\ConvOneThreeTarget{(\layersep-0 * \shift, 0+0.125, 0 * \depth)};
    

    \def\ConvTwoOneTarget{(2*\layersep-1 * \shift, 0+0.125, -1 * \depth)};
    \def\ConvTwoTwoTarget{(2*\layersep-0 * \shift, 0+0.125, -0 * \depth)};

\tikzset{
  >=latex, %
  convfilter/.style={thin, draw opacity=0.4},%
  hv/.style={to path={-| (\tikztotarget) \tikztonodes}}
}

    
    \filldraw[fill=layergray1, opacity=0.6, draw=black] (0.0 * \shift, 0, 0.0 * \depth) rectangle ++(\layerwidth, \layerheight, 0);

    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (0.0 * \shift, \i*\filtersize, 0.0 * \depth) -- (0.0 * \shift + \layerwidth,\i*\filtersize,0.0 * \depth);
    }
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (0.0 * \shift + \i*\filtersize, 0+\layerheight, 0.0 * \depth) -- (0.0 * \shift + \i*\filtersize,0,0.0 * \depth);
    }
    

    
        
    \node[scale=0.9,inner sep=0pt, anchor=center] at (+0.3 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4-0.6, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.3 * \depth+0.13333 * \depth){\footnotesize $\circledast$};
    
    \filldraw[fill=layergray2, opacity=0.6, draw=black] (-1.0 * \shift, 0, -1.0 * \depth) rectangle ++(\layerwidth, \layerheight, 0);

    



    \draw[convfilter, fill opacity=0] (0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0, 0.6 * \depth+0.13333 * \depth) rectangle ++(\filtersize*3, \filtersize*1.5, 0.0);
    \draw[convfilter] (0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2+1.5*\filtersize, 0+\yConvOneOne+\filtersize/2+0.0, 0.6 * \depth+0.13333 * \depth) -- (0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2+1.5*\filtersize, 0+\yConvOneOne+\filtersize/2+0.0+1.5*\filtersize, 0.6 * \depth+0.13333 * \depth) {};
    \node[scale=0.9,inner sep=0pt, anchor=center] at (0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.6 * \depth+0.13333 * \depth){\tiny 0};
    \node[scale=0.9,inner sep=0pt, anchor=center] at (0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize + 0.2+1.5*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.6 * \depth+0.13333 * \depth){\tiny -1};

    
    
    \draw[convfilter, fill opacity=0.75, fill=white] (-0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0, 0 * \depth+0.13333 * \depth) rectangle ++(\filtersize*3, \filtersize*1.5, 0.0);
    \draw[convfilter] (0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2+1.5*\filtersize, 0+\yConvOneOne+\filtersize/2+0.0, 0 * \depth+0.13333 * \depth) -- (0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2+1.5*\filtersize, 0+\yConvOneOne+\filtersize/2+0.0+1.5*\filtersize, 0 * \depth+0.13333 * \depth) {};
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0 * \depth+0.13333 * \depth){\tiny 1};
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize + 0.2+1.5*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0 * \depth+0.13333 * \depth){\tiny 0};


    
    


    
    \draw[convfilter, fill opacity=0.75, fill=white] (-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0, -1 * \depth-0.13333 * \depth) rectangle ++(\filtersize*3, \filtersize*1.5, 0.0);
    \draw[convfilter] (-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2+1.5*\filtersize, 0+\yConvOneOne+\filtersize/2+0.0, -1 * \depth-0.13333 * \depth) -- (-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2+1.5*\filtersize, 0+\yConvOneOne+\filtersize/2+0.0+1.5*\filtersize, -1 * \depth-0.13333 * \depth) {};
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1 * \depth-0.13333 * \depth){\tiny -1};
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize + 0.2+1.5*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1 * \depth-0.13333 * \depth){\tiny 0};

    \node[scale=0.9,inner sep=0pt, anchor=center] at (-1.3 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4-0.6, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.3 * \depth-0.13333 * \depth){\footnotesize $\circledast$};

    \draw[convfilter, fill opacity=0.75, fill=white] (-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0, -1.6 * \depth-0.13333 * \depth) rectangle ++(\filtersize*3, \filtersize*1.5, 0.0);
    \draw[convfilter] (-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2+1.5*\filtersize, 0+\yConvOneOne+\filtersize/2+0.0, -1.6 * \depth-0.13333 * \depth) -- (-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.2+1.5*\filtersize, 0+\yConvOneOne+\filtersize/2+0.0+1.5*\filtersize, -1.6 * \depth-0.13333 * \depth) {};
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.6 * \depth-0.13333 * \depth){\tiny 0};
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize + 0.2+1.5*\filtersize+0.2, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.6 * \depth-0.13333 * \depth){\tiny 1};

    



    

    
    

    





    
    \filldraw[fill=layergray1, opacity=0.6, draw=black] (\layersep - 0 * \shift, 0, -0 * \depth) rectangle ++(\layerwidth, \layerheight, 0);
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (\layersep+0.0 * \shift, \i*\filtersize, 0.0 * \depth) -- (\layersep+0.0 * \shift + \layerwidth,\i*\filtersize,0.0 * \depth);
    }
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (\layersep+0.0 * \shift + \i*\filtersize, 0+\layerheight, 0.0 * \depth) -- (\layersep+0.0 * \shift + \i*\filtersize,0,0.0 * \depth);
    }




    \draw[convfilter, fill opacity=0.75, fill=white] (\layersep+0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, 0.6 * \depth+0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[inner sep=0pt, anchor=center] at (\layersep+0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.6 * \depth+0.13333 * \depth){\tiny 1};

    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep+0.3 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4-0.5, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.3 * \depth+0.13333 * \depth){\footnotesize $\circledast$};

    \draw[convfilter, fill opacity=0.75, fill=white] (\layersep-0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, 0 * \depth+0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[inner sep=0pt, anchor=center] at (\layersep-0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, +0 * \depth+0.13333 * \depth){\tiny -1};
    

    \draw[convfilter, fill opacity=0.75, fill=white] (\layersep-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, -1 * \depth-0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1 * \depth-0.13333 * \depth){\tiny .5};

     \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep-1.3 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4-0.5, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.3 * \depth-0.13333 * \depth){\footnotesize $\circledast$};

    \draw[convfilter, fill opacity=0.75, fill=white] (\layersep-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, -1.6 * \depth-0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.6 * \depth-0.13333 * \depth){\tiny .5};
    



    
    
    

    \filldraw[fill=layergray2, opacity=0.6, draw=black] (\layersep - 1 * \shift, 0, -1 * \depth) rectangle ++(\layerwidth, \layerheight, 0);



    
    \filldraw[fill=layergray1, opacity=0.6, draw=black] (2 * \layersep - 0 * \shift, 0, -0 * \depth) rectangle ++(\layerwidth, \layerheight, 0);
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (2*\layersep+0.0 * \shift, \i*\filtersize, 0.0 * \depth) -- (2*\layersep+0.0 * \shift + \layerwidth,\i*\filtersize,0.0 * \depth);
    }
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (2*\layersep+0.0 * \shift + \i*\filtersize, 0+\layerheight, 0.0 * \depth) -- (2*\layersep+0.0 * \shift + \i*\filtersize,0,0.0 * \depth);
    }

        
    \filldraw[fill=layergray2, opacity=0.6, draw=black] (2 * \layersep - 1 * \shift, 0, -1 * \depth) rectangle ++(\layerwidth, \layerheight, 0);

    
    


    \filldraw[fill=colorSchemeOne, opacity=0.6, draw=black] (2.85 * \layersep - 0 * \shift, 2*\filtersize, -0 * \depth) rectangle ++(\filtersize, \filtersize, 0);



    \draw[convfilter, arrows={->[gray!80!black]}] (2 * \layersep -0 * \shift + \layerwidth, \layerheight/2, -0 * \depth) -- (2.85 * \layersep - 0 * \shift, \layerheight/2, -0 * \depth) node[pos=0.5, gray!60!black,yshift=0] {\contour{white}{\tiny \begin{tabular}{c} GAP \end{tabular}}};

    \draw[convfilter, arrows={->[gray!80!black]}] (2 * \layersep -1 * \shift + \layerwidth, \layerheight/2, -1 * \depth) -- (2.85 * \layersep - 1 * \shift, \layerheight/2, -1 * \depth) node[pos=0.5, gray!60!black,yshift=0] {\contour{white}{\tiny \begin{tabular}{c} GAP \end{tabular}}};

    \filldraw[fill=colorSchemeTwo, opacity=0.6, draw=black] (2.85 * \layersep - 1 * \shift, 2*\filtersize, -1 * \depth) rectangle ++(\filtersize, \filtersize, 0);

    \node[scale=0.9,inner sep=0pt, anchor=center, colorSchemeOne] at (2.85 * \layersep - 0 * \shift+\filtersize/2, 2*\filtersize+\filtersize+0.2, -0 * \depth){\tiny output 1};

    \node[scale=0.9,inner sep=0pt, anchor=center, colorSchemeTwo] at (2.85 * \layersep - 1 * \shift+\filtersize/2, 2*\filtersize-0.2, -1 * \depth){\tiny output 2};

\end{tikzpicture}


==> figures/toy_example/toy_barplot.tex <==
    \begin{tikzpicture}[every node/.style={font=\sffamily}]
    \sffamily
    \scriptsize
\def\yscale{0.0001}
\def\ticklabely{0.00cm};
\def\setuponey{0.4};
\def\setuptwoy{0.0};

\def\myxmin{0};
\def\myxmax{2};
\def\myymin{-0.3};
\def\myymax{0.4};

\def\centergroupone{0.5};
\def\centergrouptwo{1.5};
\def\centergroupthree{2.5};
\def\centergroupfour{3.5};
\def\centergroupfive{4.5};
\def\centergroupsix{5.5};
\def\centergroupseven{6.5};

\def\bardistance{0.3};
\def\barwidth{0.225};
\def\mymarkeroffsety{0.05}
    
\begin{axis}[
    axis lines=middle,
    xmin=\myxmin-0.55, xmax=\myxmax,
    ymin=\myymin-0.2, ymax=\myymax, %
    xtick=\empty, ytick=\empty,
    axis line style={draw=none},
    tick style={draw=none},
    height=3.3cm, 
    width=3.5cm,
]

\draw[-] (\myxmin,\myymin-0.004) -- (\myxmin,0.3+0.0015);
\draw[-] (\myxmin,1.45) -- (\myxmin,1.45) node[xshift=-0.7cm, anchor=center, rotate=90] {\scriptsize QUBA Score};
\draw[-] (\myxmin,\myymin) -- (\myxmax,\myymin);


\draw[-] (\myxmin,0.0) -- (\myxmin-0,0.00) node[left=\ticklabely,xshift=-0.2em] {\tiny 0};
\draw[-] (\myxmin,0.3) -- (\myxmin-0,0.3) node[left=\ticklabely,xshift=-0.2em] {\tiny 0.3};
\draw[-] (\myxmin,-0.3) -- (\myxmin-0,-0.3) node[left=\ticklabely,xshift=-0.2em] {\tiny -0.3};

\draw[-] ([yshift=-0.25cm]+1.0,\myymin) -- ([yshift=0.cm]+1.0,\myymin);


\draw[-] (\centergroupone,\myymin) -- (\centergroupone,\myymin) node[below=\ticklabely,yshift=-0.2em] {\tiny {class 1}};
\draw[-] (\centergrouptwo,\myymin) -- (\centergrouptwo,\myymin) node[below=\ticklabely,yshift=-0.2em] {\tiny {class 2}};




\draw[fill=colorSchemeOne, draw=colorSchemeOne!100] (\centergroupone-0.5*\bardistance-\barwidth/2,0+0.005) rectangle (\centergroupone-0.5*\bardistance+\barwidth/2,0.12);

\draw[-] (\centergroupone-0.5*\bardistance,0.12-0.046) -- (\centergroupone-0.5*\bardistance,0.12+0.046) node[xshift=+0.8em, yshift=+0.4em, color=colorSchemeOne, opacity=1.0] {\tiny {output 1}};


\draw[fill=colorSchemeTwo, draw=colorSchemeTwo!100] (\centergroupone+0.5*\bardistance-\barwidth/2,0-0.005) rectangle (\centergroupone+0.5*\bardistance+\barwidth/2,-0.12);

\draw[-] (\centergroupone+0.5*\bardistance,-0.12+0.046) -- (\centergroupone+0.5*\bardistance,-0.12-0.046) node[xshift=-0.2em, yshift=-0.4em, color=colorSchemeTwo, opacity=1.0] {\tiny {output 2}};



\draw[fill=colorSchemeOne, draw=colorSchemeOne!100] (\centergrouptwo-0.5*\bardistance-\barwidth/2,0-0.005) rectangle (\centergrouptwo-0.5*\bardistance+\barwidth/2,-0.24);

\draw[-] (\centergrouptwo -0.5*\bardistance,-0.24-0.046) -- (\centergrouptwo-0.5*\bardistance,-0.24+0.046);

\draw[fill=colorSchemeTwo, draw=colorSchemeTwo!100] (\centergrouptwo+0.5*\bardistance-\barwidth/2,0+0.005) rectangle (\centergrouptwo+0.5*\bardistance+\barwidth/2,0.24);

\draw[-] (\centergrouptwo+0.5*\bardistance,0.24-0.046) -- (\centergrouptwo+0.5*\bardistance,0.24+0.046);










\draw[-] (\myxmin,\myymin) -- (\myxmax,\myymin);

\draw[very thin, -, draw opacity=0.5] (\myxmin,0.3) -- (\myxmax,0.3);
\draw[very thin, -, draw opacity=0.5] (\myxmin,0.0) -- (\myxmax,0.0);
\draw[very thin, -, draw opacity=0.5] (\myxmax,-0.3) -- (\myxmax,0.3);

\end{axis}





    \end{tikzpicture}


==> figures/toy_example/toy_lenet.tex <==
\begin{tikzpicture}[scale = 0.75]%
    \sffamily
    \scriptsize

    \colorlet{layergray2}{gray!60!black}{0.5}
    \colorlet{layergray1}{black!15}{0.5}
    \def\layersep{2.85}  %
    \def\layerwidth{1.25} %
    \def\layerheight{1.25}  %
    \def\depth{-1.1}      %
    \def\shift{-0.6}      %
    \def\filtersize{0.25};
    \def\xConvOneOne{0.0};
    \def\yConvOneOne{0.0};
    \def\xConvOneTwo{0};
    \def\yConvOneTwo{\layerwidth-\filtersize-\filtersize-0.02};
    \def\xConvTwoOne{0.0};
    \def\yConvTwoOne{0.0};
    \def\xConvTwoTwo{0.0};
    \def\yConvTwoTwo{\layerwidth-\filtersize-\filtersize-0.02};

    \def\ConvOneOneTarget{(\layersep-1 * \shift, 0+0.125, -1 * \depth)};
    \def\ConvOneTwoTarget{(\layersep-0 * \shift, 0+1.225, -0 * \depth)};
    \def\ConvOneThreeTarget{(\layersep-0 * \shift, 0+0.125, 0 * \depth)};
    

    \def\ConvTwoOneTarget{(2*\layersep-1 * \shift, 0+0.125, -1 * \depth)};
    \def\ConvTwoTwoTarget{(2*\layersep-0 * \shift, 0+0.125, -0 * \depth)};

\tikzset{
  >=latex, %
  convfilter/.style={thin, draw opacity=0.4},%
  hv/.style={to path={-| (\tikztotarget) \tikztonodes}}
}

    
    \filldraw[fill=layergray1, opacity=0.6, draw=black] (0.5 * \shift, 0, 0.5 * \depth) rectangle ++(\layerwidth, \layerheight, 0);

    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (0.5 * \shift, \i*\filtersize, 0.5 * \depth) -- (0.5 * \shift + \layerwidth,\i*\filtersize,0.5 * \depth);
    }
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (0.5 * \shift + \i*\filtersize, 0+\layerheight, 0.5 * \depth) -- (0.5 * \shift + \i*\filtersize,0,0.5 * \depth);
    }
    

    
        
    
    \filldraw[fill=layergray2, opacity=0.6, draw=black] (-0.5 * \shift, 0, -0.5 * \depth) rectangle ++(\layerwidth, \layerheight, 0);

    


    

    \node[scale=0.9,inner sep=0pt, anchor=center] at (0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4-0.5, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.6 * \depth+0.13333 * \depth){\footnotesize $\circledast$};

    \draw[convfilter, fill opacity=0.75, fill=white] (1.2 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, 1.2 * \depth+0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (1.2 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 1.2 * \depth+0.13333 * \depth){\tiny 5};

    \draw[convfilter, fill opacity=0.75, fill=white] (0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, 0.6 * \depth+0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.6 * \depth+0.13333 * \depth){\tiny 0};

    \draw[convfilter, fill opacity=0.75, fill=white] (0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, 0 * \depth+0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, +0 * \depth+0.13333 * \depth){\tiny 5};
    


    \node[scale=0.9,inner sep=0pt, anchor=center] at (-1.6 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4-0.5, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.6 * \depth-0.13333 * \depth){\footnotesize $\circledast$};


    \draw[convfilter, fill opacity=0.75, fill=white] (-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, -1 * \depth-0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1 * \depth-0.13333 * \depth){\tiny 0};

    \draw[convfilter, fill opacity=0.75, fill=white] (-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, -1.6 * \depth-0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.6 * \depth-0.13333 * \depth){\tiny 19};

    \draw[convfilter, fill opacity=0.75, fill=white] (-2.2 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, -2.2 * \depth-0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (-2.2 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -2.2 * \depth-0.13333 * \depth){\tiny 0};



    

    \filldraw[fill=layergray1, opacity=0.6, draw=black] (-1.5 * \shift, 0, -1.5 * \depth) rectangle ++(\layerwidth, \layerheight, 0);
    
    

    





    
    \filldraw[fill=layergray1, opacity=0.6, draw=black] (\layersep - 0 * \shift, 0, -0 * \depth) rectangle ++(\layerwidth, \layerheight, 0);
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (\layersep+0.0 * \shift, \i*\filtersize, 0.0 * \depth) -- (\layersep+0.0 * \shift + \layerwidth,\i*\filtersize,0.0 * \depth);
    }
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (\layersep+0.0 * \shift + \i*\filtersize, 0+\layerheight, 0.0 * \depth) -- (\layersep+0.0 * \shift + \i*\filtersize,0,0.0 * \depth);
    }


    

    \draw[convfilter, fill opacity=0.75, fill=white] (\layersep+0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, 0.6 * \depth+0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep+0.6 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.6 * \depth+0.13333 * \depth){\tiny -4};

    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep+0.3 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4-0.5, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, 0.3 * \depth+0.13333 * \depth){\footnotesize $\circledast$};

    \draw[convfilter, fill opacity=0.75, fill=white] (\layersep-0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, 0 * \depth+0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep-0 * \shift+0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, +0 * \depth+0.13333 * \depth){\tiny 18};

    \draw[convfilter, fill opacity=0.75, fill=white] (\layersep-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, -1 * \depth-0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep-1 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1 * \depth-0.13333 * \depth){\tiny 4};

    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep-1.3 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4-0.5, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.3 * \depth-0.13333 * \depth){\footnotesize $\circledast$};

    \draw[convfilter, fill opacity=0.75, fill=white] (\layersep-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0, -1.6 * \depth-0.13333 * \depth) rectangle ++(\filtersize*1.5, \filtersize*1.5, 0.0);
    \node[scale=0.9,inner sep=0pt, anchor=center] at (\layersep-1.6 * \shift-0.13333 * \shift + \xConvOneOne + 6*\filtersize+0.75*\filtersize+0.4, 0+\yConvOneOne+\filtersize/2+0.0+0.75*\filtersize, -1.6 * \depth-0.13333 * \depth){\tiny -18};


    


    
    
    

    \filldraw[fill=layergray2, opacity=0.6, draw=black] (\layersep - 1 * \shift, 0, -1 * \depth) rectangle ++(\layerwidth, \layerheight, 0);



    
    \filldraw[fill=layergray1, opacity=0.6, draw=black] (2 * \layersep - 0 * \shift, 0, -0 * \depth) rectangle ++(\layerwidth, \layerheight, 0);
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (2*\layersep+0.0 * \shift, \i*\filtersize, 0.0 * \depth) -- (2*\layersep+0.0 * \shift + \layerwidth,\i*\filtersize,0.0 * \depth);
    }
    \foreach \i in {0,...,4} {
        \draw [very thin,gray,draw opacity=0.5,dash pattern=on 1pt off 1pt] (2*\layersep+0.0 * \shift + \i*\filtersize, 0+\layerheight, 0.0 * \depth) -- (2*\layersep+0.0 * \shift + \i*\filtersize,0,0.0 * \depth);
    }

        
    \filldraw[fill=layergray2, opacity=0.6, draw=black] (2 * \layersep - 1 * \shift, 0, -1 * \depth) rectangle ++(\layerwidth, \layerheight, 0);

    
    


    \filldraw[fill=colorSchemeOne, opacity=0.6, draw=black] (2.85 * \layersep - 0 * \shift, 2*\filtersize, -0 * \depth) rectangle ++(\filtersize, \filtersize, 0);


    \draw[convfilter, arrows={->[gray!80!black]}] (2 * \layersep -0 * \shift + \layerwidth, \layerheight/2, -0 * \depth) -- (2.85 * \layersep - 0 * \shift, \layerheight/2, -0 * \depth) node[pos=0.5, gray!60!black,yshift=0] {\contour{white}{\tiny \begin{tabular}{c} GAP \end{tabular}}};

    \draw[convfilter, arrows={->[gray!80!black]}] (2 * \layersep -1 * \shift + \layerwidth, \layerheight/2, -1 * \depth) -- (2.85 * \layersep - 1 * \shift, \layerheight/2, -1 * \depth) node[pos=0.5, gray!60!black,yshift=0] {\contour{white}{\tiny \begin{tabular}{c} GAP \end{tabular}}};
    

    \filldraw[fill=colorSchemeTwo, opacity=0.6, draw=black] (2.85 * \layersep - 1 * \shift, 2*\filtersize, -1 * \depth) rectangle ++(\filtersize, \filtersize, 0);

    \node[scale=0.9,inner sep=0pt, anchor=center, colorSchemeOne] at (2.85 * \layersep - 0 * \shift+\filtersize/2, 2*\filtersize+\filtersize+0.2, -0 * \depth){\tiny output 1};

    \node[scale=0.9,inner sep=0pt, anchor=center, colorSchemeTwo] at (2.85 * \layersep - 1 * \shift+\filtersize/2, 2*\filtersize-0.2, -1 * \depth){\tiny output 2};
    

\end{tikzpicture}

